High-resolution spectroscopy of extremely metal-poor stars in the least evolved galaxies: Bootes II

We present high-resolution Magellan/MIKE spectra of the four brightest confirmed red giant stars in the ultra-faint dwarf galaxy Bootes II (Boo II). These stars all inhabit the metal-poor tail of the Boo II metallicity distribution function. The chemical abundance pattern of all detectable elements in these stars is consistent with that of the Galactic halo. However, all four stars have undetectable amounts of neutron-capture elements Sr and Ba, with upper limits comparable to the lowest ever detected in the halo or in other dwarf galaxies. One star exhibits significant radial velocity variations over time, suggesting it to be in a binary system. Its variable velocity has likely increased past determinations of the Boo II velocity dispersion. Our four stars span a limited metallicity range, but their enhanced {\alpha}-abundances and low neutron-capture abundances are consistent with the interpretation that Boo II has been enriched by very few generations of stars. The chemical abundance pattern in Boo II confirms the emerging trend that the faintest dwarf galaxies have neutron-capture abundances distinct from the halo, suggesting the dominant source of neutron-capture elements in halo stars may be different than in ultra-faint dwarfs.

==> ew.tex <==
\begin{deluxetable*}{llrrrrrrrrrr}
\tablecolumns{12}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tabletypesize{\tiny}
\tablecaption{Equivalent Widths\label{tbl:ew}}
\tablehead{\colhead{El.} & \colhead{$\lambda$} & \colhead{$\chi$} & \colhead{$\log gf$} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon$ (dex)} & \colhead{EW (m\AA)} & \colhead{$\log \epsilon$ (dex)}\\
\colhead{} & \colhead{(\AA)} & \colhead{(eV)} & \colhead{(dex)} & \multicolumn{2}{c}{\StarA} & \multicolumn{2}{c}{\StarB} & \multicolumn{2}{c}{\StarC} & \multicolumn{2}{c}{\StarD}}
\startdata
CH     & 4313     &\nodata&\nodata   &     syn &    5.97 &     syn &    6.10 &     syn &    5.91 &     syn &    6.06 \\
CH     & 4323     &\nodata&\nodata   &     syn &    5.97 &     syn &    6.15 &     syn &    5.91 &     syn &    6.06 \\
Na\,I  &  5889.95 &  0.00 & $  0.11$ &   151.4 &    3.84 &   186.0 &    4.09 &   168.2 &    3.96 &   133.4 &    3.68 \\
Na\,I  &  5895.92 &  0.00 & $ -0.19$ &   142.7 &    4.00 &   160.3 &    4.04 &   144.2 &    3.89 &   114.5 &    3.66 \\
Mg\,I  &  4571.10 &  0.00 & $ -5.69$ & \nodata & \nodata &    67.2 &    5.56 &    39.1 &    5.25 & \nodata & \nodata \\
Mg\,I  &  4702.99 &  4.33 & $ -0.38$ &    55.5 &    5.05 &    84.5 &    5.40 &    67.2 &    5.19 &    48.7 &    5.01 \\
Mg\,I  &  5172.68 &  2.71 & $ -0.45$ &   184.0 &    5.29 &   192.1 &    5.24 &   161.5 &    4.97 &   154.7 &    5.00 \\
Mg\,I  &  5183.60 &  2.72 & $ -0.24$ &   174.2 &    4.99 &   237.1 &    5.39 &   193.9 &    5.12 &   159.7 &    4.86 \\
Mg\,I  &  5528.40 &  4.34 & $ -0.50$ &    61.4 &    5.27 &    64.3 &    5.23 &    43.8 &    4.96 &    46.2 &    5.10 \\
Al\,I  &  3961.52 &  0.01 & $ -0.34$ &    97.3 &    2.63 &   105.6 &    2.64 &    90.1 &    2.41 & \nodata & \nodata \\
Al\,I  &  3944.00 &  0.00 & $ -0.62$ &     syn &    2.69 &     syn &    2.92 &     syn &    2.53 &     syn & $<$4.28 \\
Si\,I  &  3905.52 &  1.91 & $ -1.09$ &     syn &    4.65 &     syn & $<$5.88 &     syn &    4.59 &     syn & $<$5.64 \\
Ca\,I  &  4226.73 &  0.00 & $  0.24$ &   197.2 &    3.89 &   252.7 &    4.14 & \nodata & \nodata & \nodata & \nodata \\
Ca\,I  &  4283.01 &  1.89 & $ -0.22$ & \nodata & \nodata &    77.6 &    4.32 &    56.5 &    4.00 & \nodata & \nodata \\
Ca\,I  &  4425.44 &  1.88 & $ -0.36$ & \nodata & \nodata &    65.8 &    4.22 & \nodata & \nodata & \nodata & \nodata \\
Ca\,I  &  4434.96 &  1.89 & $ -0.01$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    51.0 &    3.85 \\
Ca\,I  &  4454.78 &  1.90 & $  0.26$ &    72.2 &    3.84 &    95.6 &    4.16 &    72.3 &    3.78 &    62.6 &    3.80 \\
Ca\,I  &  4455.89 &  1.90 & $ -0.53$ & \nodata & \nodata & \nodata & \nodata &    41.2 &    4.05 & \nodata & \nodata \\
Ca\,I  &  5588.76 &  2.52 & $  0.21$ & \nodata & \nodata &    58.2 &    4.19 & \nodata & \nodata & \nodata & \nodata \\
Ca\,I  &  5594.47 &  2.52 & $  0.10$ &    36.7 &    4.03 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca\,I  &  6122.22 &  1.89 & $ -0.32$ & \nodata & \nodata &    74.7 &    4.23 &    48.9 &    3.88 & \nodata & \nodata \\
Ca\,I  &  6162.17 &  1.90 & $ -0.09$ & \nodata & \nodata &    79.4 &    4.09 &    58.6 &    3.82 & \nodata & \nodata \\
Ca\,I  &  6439.07 &  2.52 & $  0.47$ &    52.6 &    3.92 &    71.6 &    4.12 &    59.8 &    3.97 & \nodata & \nodata \\
Sc\,II & 4246.82  &  0.32 & $  0.24$ &     syn &    0.59 &     syn &    0.12 &     syn &    0.08 &     syn &    0.39 \\
Sc\,II & 4314.08  &  0.62 & $ -0.10$ &     syn &    0.69 &     syn &    0.22 &     syn &    0.13 &     syn & $<$0.78 \\
Sc\,II & 4324.99  &  0.59 & $ -0.44$ &     syn &    0.49 &     syn &    0.42 &     syn &  $-0.07$&     syn &    0.34 \\
Sc\,II & 4400.38  &  0.61 & $ -0.54$ & \nodata & \nodata &     syn &    0.42 & \nodata & \nodata & \nodata & \nodata \\
Sc\,II & 4415.54  &  0.59 & $ -0.67$ & \nodata & \nodata &     syn &    0.42 & \nodata & \nodata & \nodata & \nodata \\
Ti\,I  &  4533.25 &  0.85 & $  0.53$ & \nodata & \nodata &    61.8 &    2.66 & \nodata & \nodata & \nodata & \nodata \\
Ti\,I  &  4991.07 &  0.84 & $  0.44$ & \nodata & \nodata &    62.6 &    2.71 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  3913.46 &  1.12 & $ -0.42$ & \nodata & \nodata &   108.8 &    2.39 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4290.22 &  1.16 & $ -0.93$ &    85.6 &    2.55 &    91.1 &    2.40 &    71.5 &    2.12 &    69.0 &    2.49 \\
Ti\,II &  4300.05 &  1.18 & $ -0.49$ &    84.8 &    2.11 &   109.9 &    2.41 &   101.5 &    2.34 &    91.0 &    2.62 \\
Ti\,II &  4337.91 &  1.08 & $ -0.96$ &    73.1 &    2.21 &    99.8 &    2.52 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4394.06 &  1.22 & $ -1.78$ & \nodata & \nodata & \nodata & \nodata &    24.8 &    2.20 & \nodata & \nodata \\
Ti\,II &  4395.03 &  1.08 & $ -0.54$ &    92.0 &    2.19 &   114.8 &    2.43 &   100.5 &    2.23 &    85.7 &    2.40 \\
Ti\,II &  4395.84 &  1.24 & $ -1.93$ & \nodata & \nodata &    35.5 &    2.51 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4399.77 &  1.24 & $ -1.19$ &    52.6 &    2.25 &    66.7 &    2.28 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4417.71 &  1.17 & $ -1.19$ & \nodata & \nodata &    74.4 &    2.33 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4443.80 &  1.08 & $ -0.72$ &    87.8 &    2.27 &   111.2 &    2.51 &    92.7 &    2.21 &    90.5 &    2.69 \\
Ti\,II &  4450.48 &  1.08 & $ -1.52$ & \nodata & \nodata &    58.3 &    2.28 &    51.9 &    2.27 & \nodata & \nodata \\
Ti\,II &  4464.45 &  1.16 & $ -1.81$ & \nodata & \nodata &    57.5 &    2.65 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  4468.52 &  1.13 & $ -0.60$ &    86.7 &    2.18 &   109.0 &    2.39 &    96.7 &    2.24 &    81.9 &    2.41 \\
Ti\,II &  4501.27 &  1.12 & $ -0.77$ &    85.9 &    2.31 &   110.8 &    2.58 &    86.4 &    2.17 &    70.1 &    2.28 \\
Ti\,II &  4533.96 &  1.24 & $ -0.53$ &    82.7 &    2.13 &   116.6 &    2.60 &    94.3 &    2.22 &    74.2 &    2.26 \\
Ti\,II &  4563.77 &  1.22 & $ -0.96$ &    74.7 &    2.38 &    86.0 &    2.35 &    64.9 &    2.07 &    70.1 &    2.57 \\
Ti\,II &  4571.97 &  1.57 & $ -0.32$ &    76.3 &    2.16 &    99.9 &    2.40 &    78.7 &    2.08 &    69.9 &    2.32 \\
Ti\,II &  4805.09 &  2.06 & $ -1.10$ & \nodata & \nodata &    38.2 &    2.63 & \nodata & \nodata & \nodata & \nodata \\
Ti\,II &  5188.69 &  1.58 & $ -1.05$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    49.8 &    2.61 \\
Ti\,II &  5226.54 &  1.57 & $ -1.26$ & \nodata & \nodata & \nodata & \nodata &    34.2 &    2.21 &    35.5 &    2.54 \\
Cr\,I  &  4254.33 &  0.00 & $ -0.11$ &    98.6 &    2.54 &   123.3 &    2.87 &   103.2 &    2.53 &    86.7 &    2.55 \\
Cr\,I  &  4274.80 &  0.00 & $ -0.22$ &   100.0 &    2.68 &   112.9 &    2.73 & \nodata & \nodata &    78.0 &    2.43 \\
Cr\,I  &  4289.72 &  0.00 & $ -0.37$ &    83.4 &    2.42 &   108.3 &    2.77 &    90.1 &    2.47 & \nodata & \nodata \\
Cr\,I  &  4646.15 &  1.03 & $ -0.74$ & \nodata & \nodata &    38.7 &    2.93 & \nodata & \nodata & \nodata & \nodata \\
Cr\,I  &  5206.04 &  0.94 & $  0.02$ &    69.1 &    2.71 &    83.1 &    2.77 &    59.2 &    2.45 &    59.4 &    2.71 \\
Cr\,I  &  5208.42 &  0.94 & $  0.16$ & \nodata & \nodata &    96.6 &    2.89 &    74.2 &    2.56 & \nodata & \nodata \\
Mn\,I  & 4030.75  &  0.00 & $ -0.48$ &     syn &    1.97 &     syn &    3.10 &     syn &    1.61 &     syn & $<$3.06 \\
Mn\,I  & 4033.06  &  0.00 & $ -0.61$ &     syn &    1.97 &     syn &    2.80 &     syn &    1.81 &     syn & $<$3.06 \\
Mn\,I  & 4034.48  &  0.00 & $ -0.81$ &     syn &    1.77 &     syn &    2.50 &     syn &    1.81 &     syn &    2.57 \\
Fe\,I  &  3827.82 &  1.56 & $  0.09$ &   155.9 &    4.85 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  3840.44 &  0.99 & $ -0.50$ &   141.4 &    4.65 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  3846.80 &  3.25 & $ -0.02$ & \nodata & \nodata &    71.1 &    4.92 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  3850.82 &  0.99 & $ -1.75$ & \nodata & \nodata & \nodata & \nodata &    77.1 &    4.30 & \nodata & \nodata \\
Fe\,I  &  3878.57 &  0.09 & $ -1.38$ &   152.8 &    4.70 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  3887.05 &  0.91 & $ -1.14$ &   105.6 &    4.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  3895.66 &  0.11 & $ -1.67$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   111.0 &    4.54 \\
Fe\,I  &  3917.18 &  0.99 & $ -2.15$ & \nodata & \nodata &    87.6 &    4.81 &    75.0 &    4.65 & \nodata & \nodata \\
Fe\,I  &  3920.26 &  0.12 & $ -1.73$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   120.0 &    4.78 \\
Fe\,I  &  3922.91 &  0.05 & $ -1.63$ &   124.2 &    4.39 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4005.24 &  1.56 & $ -0.58$ & \nodata & \nodata & \nodata & \nodata &    98.1 &    4.25 & \nodata & \nodata \\
Fe\,I  &  4007.27 &  2.76 & $ -1.28$ & \nodata & \nodata &    37.6 &    4.99 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4014.53 &  3.05 & $ -0.59$ & \nodata & \nodata &    54.0 &    4.91 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4021.87 &  2.76 & $ -0.73$ & \nodata & \nodata & \nodata & \nodata &    46.3 &    4.66 & \nodata & \nodata \\
Fe\,I  &  4032.63 &  1.49 & $ -2.38$ & \nodata & \nodata &    40.0 &    4.68 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4063.59 &  1.56 & $  0.06$ &   131.7 &    4.46 & \nodata & \nodata & \nodata & \nodata &   125.7 &    4.55 \\
Fe\,I  &  4067.98 &  3.21 & $ -0.47$ &    46.1 &    4.93 &    40.9 &    4.73 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4071.74 &  1.61 & $ -0.01$ &   119.0 &    4.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4132.06 &  1.61 & $ -0.68$ &    91.7 &    4.31 &   123.3 &    4.84 &   102.0 &    4.46 &    90.0 &    4.57 \\
Fe\,I  &  4132.90 &  2.85 & $ -1.01$ & \nodata & \nodata &    43.6 &    4.91 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4134.68 &  2.83 & $ -0.65$ & \nodata & \nodata &    50.1 &    4.64 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4143.41 &  3.05 & $ -0.20$ & \nodata & \nodata &    69.0 &    4.78 & \nodata & \nodata &    45.3 &    4.61 \\
Fe\,I  &  4143.87 &  1.56 & $ -0.51$ &   113.3 &    4.62 &   136.2 &    4.88 &   117.4 &    4.61 &    99.2 &    4.57 \\
Fe\,I  &  4147.67 &  1.48 & $ -2.07$ & \nodata & \nodata &    62.9 &    4.74 &    59.3 &    4.77 & \nodata & \nodata \\
Fe\,I  &  4152.17 &  0.96 & $ -3.23$ & \nodata & \nodata &    41.0 &    4.93 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4154.50 &  2.83 & $ -0.69$ & \nodata & \nodata & \nodata & \nodata &    46.1 &    4.68 & \nodata & \nodata \\
Fe\,I  &  4154.81 &  3.37 & $ -0.40$ & \nodata & \nodata &    29.2 &    4.61 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4156.80 &  2.83 & $ -0.81$ & \nodata & \nodata &    47.1 &    4.75 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4175.64 &  2.85 & $ -0.83$ & \nodata & \nodata &    54.0 &    4.91 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4181.76 &  2.83 & $ -0.37$ & \nodata & \nodata &    68.7 &    4.69 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4187.04 &  2.45 & $ -0.51$ &    61.9 &    4.40 &    97.9 &    4.99 &    55.1 &    4.22 &    67.1 &    4.69 \\
Fe\,I  &  4187.80 &  2.42 & $ -0.51$ & \nodata & \nodata & \nodata & \nodata &    73.7 &    4.53 & \nodata & \nodata \\
Fe\,I  &  4191.43 &  2.47 & $ -0.67$ & \nodata & \nodata &    80.9 &    4.81 &    70.0 &    4.67 &    56.7 &    4.66 \\
Fe\,I  &  4195.33 &  3.33 & $ -0.49$ & \nodata & \nodata & \nodata & \nodata &    35.3 &    4.84 & \nodata & \nodata \\
Fe\,I  &  4199.10 &  3.05 & $  0.16$ &    63.8 &    4.45 &    89.1 &    4.84 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4202.03 &  1.49 & $ -0.69$ &   106.7 &    4.54 &   127.7 &    4.79 &   109.6 &    4.50 &    92.9 &    4.51 \\
Fe\,I  &  4216.18 &  0.00 & $ -3.36$ &    66.0 &    4.57 &    90.6 &    4.86 &    82.0 &    4.80 & \nodata & \nodata \\
Fe\,I  &  4222.21 &  2.45 & $ -0.91$ & \nodata & \nodata &    77.1 &    4.94 &    48.9 &    4.51 & \nodata & \nodata \\
Fe\,I  &  4227.43 &  3.33 & $  0.27$ & \nodata & \nodata &    75.3 &    4.73 &    56.1 &    4.44 &    45.4 &    4.43 \\
Fe\,I  &  4233.60 &  2.48 & $ -0.58$ &    69.0 &    4.64 &    82.8 &    4.76 &    63.7 &    4.47 &    62.0 &    4.68 \\
Fe\,I  &  4238.81 &  3.40 & $ -0.23$ & \nodata & \nodata &    39.8 &    4.67 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4250.12 &  2.47 & $ -0.38$ &    61.2 &    4.27 &    87.1 &    4.64 &    67.0 &    4.32 & \nodata & \nodata \\
Fe\,I  &  4250.79 &  1.56 & $ -0.71$ &    96.6 &    4.38 &   125.8 &    4.83 &   116.2 &    4.75 &    92.6 &    4.59 \\
Fe\,I  &  4260.47 &  2.40 & $  0.08$ &   100.5 &    4.56 &   114.0 &    4.67 &    92.9 &    4.31 &    85.8 &    4.45 \\
Fe\,I  &  4271.15 &  2.45 & $ -0.34$ &    91.5 &    4.83 & \nodata & \nodata &    94.9 &    4.83 &    75.3 &    4.69 \\
Fe\,I  &  4271.76 &  1.49 & $ -0.17$ &   132.7 &    4.58 & \nodata & \nodata & \nodata & \nodata &   118.9 &    4.55 \\
Fe\,I  &  4282.40 &  2.18 & $ -0.78$ &    61.2 &    4.36 &    85.4 &    4.69 &    83.6 &    4.74 & \nodata & \nodata \\
Fe\,I  &  4325.76 &  1.61 & $  0.01$ & \nodata & \nodata & \nodata & \nodata &   129.6 &    4.35 &   131.2 &    4.68 \\
Fe\,I  &  4337.05 &  1.56 & $ -1.70$ &    64.9 &    4.65 &    86.0 &    4.89 &    68.1 &    4.63 & \nodata & \nodata \\
Fe\,I  &  4352.73 &  2.22 & $ -1.29$ &    61.0 &    4.90 &    68.7 &    4.89 &    50.3 &    4.65 & \nodata & \nodata \\
Fe\,I  &  4375.93 &  0.00 & $ -3.00$ &    81.0 &    4.51 &   112.0 &    4.95 &    85.7 &    4.49 & \nodata & \nodata \\
Fe\,I  &  4383.55 &  1.48 & $  0.20$ &   176.7 &    4.77 & \nodata & \nodata & \nodata & \nodata &   138.7 &    4.45 \\
Fe\,I  &  4404.75 &  1.56 & $ -0.15$ &   128.5 &    4.52 & \nodata & \nodata &   128.1 &    4.40 & \nodata & \nodata \\
Fe\,I  &  4415.12 &  1.61 & $ -0.62$ &   110.1 &    4.64 &   130.3 &    4.84 &   120.0 &    4.75 &    99.8 &    4.69 \\
Fe\,I  &  4427.31 &  0.05 & $ -2.92$ &    91.6 &    4.72 &   113.6 &    4.96 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4430.61 &  2.22 & $ -1.66$ & \nodata & \nodata &    35.9 &    4.68 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4442.34 &  2.20 & $ -1.23$ &    69.3 &    4.97 &    69.7 &    4.81 &    59.9 &    4.72 & \nodata & \nodata \\
Fe\,I  &  4443.19 &  2.86 & $ -1.04$ & \nodata & \nodata &    38.3 &    4.83 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4447.72 &  2.22 & $ -1.34$ & \nodata & \nodata &    62.1 &    4.80 &    36.2 &    4.44 & \nodata & \nodata \\
Fe\,I  &  4459.12 &  2.18 & $ -1.28$ &    68.0 &    4.97 &    66.4 &    4.78 &    53.9 &    4.64 & \nodata & \nodata \\
Fe\,I  &  4461.65 &  0.09 & $ -3.19$ & \nodata & \nodata &   107.4 &    5.11 &    79.7 &    4.64 &    70.5 &    4.84 \\
Fe\,I  &  4466.55 &  2.83 & $ -0.60$ &    52.3 &    4.72 &    73.9 &    4.98 &    39.7 &    4.45 & \nodata & \nodata \\
Fe\,I  &  4476.02 &  2.85 & $ -0.82$ &    51.8 &    4.96 &    56.3 &    4.90 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4489.74 &  0.12 & $ -3.90$ & \nodata & \nodata &    65.2 &    4.98 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4494.56 &  2.20 & $ -1.14$ & \nodata & \nodata &    83.0 &    4.97 & \nodata & \nodata &    49.6 &    4.67 \\
Fe\,I  &  4528.61 &  2.18 & $ -0.82$ &    65.5 &    4.45 &    96.7 &    4.91 &    66.8 &    4.40 &    55.3 &    4.44 \\
Fe\,I  &  4531.15 &  1.48 & $ -2.10$ &    38.0 &    4.46 &    71.2 &    4.87 &    60.6 &    4.78 & \nodata & \nodata \\
Fe\,I  &  4602.94 &  1.49 & $ -2.21$ & \nodata & \nodata &    70.9 &    4.97 &    32.9 &    4.41 & \nodata & \nodata \\
Fe\,I  &  4859.74 &  2.88 & $ -0.76$ &    44.1 &    4.77 &    46.4 &    4.68 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4871.32 &  2.87 & $ -0.36$ &    46.1 &    4.39 &    83.9 &    4.92 &    46.9 &    4.35 &    53.0 &    4.65 \\
Fe\,I  &  4872.14 &  2.88 & $ -0.57$ & \nodata & \nodata &    78.7 &    5.04 &    41.2 &    4.47 &    44.4 &    4.71 \\
Fe\,I  &  4890.76 &  2.88 & $ -0.39$ & \nodata & \nodata &    81.4 &    4.91 &    46.2 &    4.37 &    50.3 &    4.64 \\
Fe\,I  &  4891.49 &  2.85 & $ -0.11$ &    86.3 &    4.86 &    96.1 &    4.88 &    55.8 &    4.22 &    56.0 &    4.44 \\
Fe\,I  &  4903.31 &  2.88 & $ -0.93$ &    33.6 &    4.74 &    49.5 &    4.90 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4918.99 &  2.85 & $ -0.34$ & \nodata & \nodata &    90.9 &    5.00 &    64.5 &    4.59 &    60.9 &    4.76 \\
Fe\,I  &  4920.50 &  2.83 & $  0.07$ &    69.3 &    4.32 &    96.1 &    4.67 &    81.5 &    4.47 & \nodata & \nodata \\
Fe\,I  &  4938.81 &  2.88 & $ -1.08$ & \nodata & \nodata &    30.0 &    4.70 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4939.69 &  0.86 & $ -3.25$ & \nodata & \nodata &    49.1 &    4.89 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  4994.13 &  0.92 & $ -2.97$ & \nodata & \nodata &    71.7 &    5.03 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5012.07 &  0.86 & $ -2.64$ & \nodata & \nodata &    80.9 &    4.80 &    49.4 &    4.38 &    44.8 &    4.56 \\
Fe\,I  &  5041.07 &  0.96 & $ -3.09$ & \nodata & \nodata & \nodata & \nodata &    41.4 &    4.80 & \nodata & \nodata \\
Fe\,I  &  5041.76 &  1.49 & $ -2.20$ & \nodata & \nodata &    58.6 &    4.71 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5079.22 &  2.20 & $ -2.10$ & \nodata & \nodata &    36.8 &    5.06 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5079.74 &  0.99 & $ -3.25$ & \nodata & \nodata &    55.1 &    5.12 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5083.34 &  0.96 & $ -2.84$ &    61.0 &    4.97 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5110.41 &  0.00 & $ -3.76$ &    71.3 &    4.98 &    88.1 &    5.03 &    72.5 &    4.87 & \nodata & \nodata \\
Fe\,I  &  5123.72 &  1.01 & $ -3.06$ & \nodata & \nodata & \nodata & \nodata &    37.7 &    4.76 & \nodata & \nodata \\
Fe\,I  &  5127.36 &  0.92 & $ -3.25$ & \nodata & \nodata &    49.2 &    4.94 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5142.93 &  0.96 & $ -3.08$ & \nodata & \nodata &    55.5 &    4.92 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5150.84 &  0.99 & $ -3.04$ & \nodata & \nodata &    62.0 &    5.01 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5166.28 &  0.00 & $ -4.12$ & \nodata & \nodata &    51.4 &    4.77 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5171.60 &  1.49 & $ -1.72$ &    69.0 &    4.59 &    86.6 &    4.71 &    72.8 &    4.56 &    62.9 &    4.68 \\
Fe\,I  &  5192.34 &  3.00 & $ -0.42$ & \nodata & \nodata &    66.0 &    4.78 & \nodata & \nodata &    42.3 &    4.64 \\
Fe\,I  &  5194.94 &  1.56 & $ -2.02$ &    53.4 &    4.69 &    83.1 &    5.02 &    55.9 &    4.65 &    33.3 &    4.48 \\
Fe\,I  &  5198.71 &  2.22 & $ -2.09$ & \nodata & \nodata &    31.1 &    4.96 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5202.34 &  2.18 & $ -1.87$ & \nodata & \nodata &    47.8 &    4.99 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5216.27 &  1.61 & $ -2.08$ & \nodata & \nodata &    78.3 &    5.05 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5225.53 &  0.11 & $ -4.75$ & \nodata & \nodata &    28.1 &    5.12 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5232.94 &  2.94 & $ -0.06$ &    60.0 &    4.39 &    88.5 &    4.75 &    64.0 &    4.39 & \nodata & \nodata \\
Fe\,I  &  5266.56 &  3.00 & $ -0.39$ &    44.9 &    4.52 &    56.7 &    4.59 & \nodata & \nodata &    46.3 &    4.68 \\
Fe\,I  &  5269.54 &  0.86 & $ -1.33$ &   134.3 &    4.89 &   146.3 &    4.78 &   125.2 &    4.54 &   111.8 &    4.71 \\
Fe\,I  &  5281.79 &  3.04 & $ -0.83$ & \nodata & \nodata &    33.7 &    4.69 &    34.8 &    4.77 & \nodata & \nodata \\
Fe\,I  &  5283.62 &  3.24 & $ -0.52$ & \nodata & \nodata &    46.8 &    4.83 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5302.30 &  3.28 & $ -0.72$ & \nodata & \nodata &    40.4 &    4.97 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5307.36 &  1.61 & $ -2.91$ & \nodata & \nodata &    26.0 &    4.97 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5324.18 &  3.21 & $ -0.10$ & \nodata & \nodata &    75.1 &    4.85 &    63.8 &    4.72 & \nodata & \nodata \\
Fe\,I  &  5328.04 &  0.92 & $ -1.47$ &   119.0 &    4.77 &   152.7 &    5.08 &   117.5 &    4.57 &    95.0 &    4.53 \\
Fe\,I  &  5328.53 &  1.56 & $ -1.85$ & \nodata & \nodata &    78.2 &    4.75 &    62.4 &    4.58 & \nodata & \nodata \\
Fe\,I  &  5339.93 &  3.27 & $ -0.72$ & \nodata & \nodata &    38.4 &    4.92 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5371.49 &  0.96 & $ -1.64$ & \nodata & \nodata &   129.5 &    4.86 &   109.6 &    4.60 &    91.8 &    4.66 \\
Fe\,I  &  5383.37 &  4.31 & $  0.65$ & \nodata & \nodata &    40.1 &    4.76 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  5397.13 &  0.92 & $ -1.98$ &   104.6 &    4.95 &   119.5 &    4.95 &   101.6 &    4.72 & \nodata & \nodata \\
Fe\,I  &  5405.77 &  0.99 & $ -1.85$ &    90.1 &    4.57 &   120.8 &    4.93 &   105.8 &    4.76 &    91.5 &    4.89 \\
Fe\,I  &  5429.70 &  0.96 & $ -1.88$ &    98.2 &    4.74 &   129.1 &    5.09 &    96.0 &    4.54 &    79.5 &    4.60 \\
Fe\,I  &  5434.52 &  1.01 & $ -2.13$ &    78.2 &    4.61 &   101.8 &    4.83 &    80.3 &    4.53 &    72.2 &    4.74 \\
Fe\,I  &  5446.92 &  0.99 & $ -1.91$ &   105.2 &    4.97 &   107.0 &    4.69 &   105.3 &    4.80 &    87.7 &    4.86 \\
Fe\,I  &  5455.61 &  1.01 & $ -2.09$ & \nodata & \nodata &   112.7 &    5.01 &    99.8 &    4.89 &    69.7 &    4.64 \\
Fe\,I  &  5497.52 &  1.01 & $ -2.83$ &    41.6 &    4.66 & \nodata & \nodata &    38.2 &    4.52 &    36.6 &    4.73 \\
Fe\,I  &  5506.78 &  0.99 & $ -2.79$ & \nodata & \nodata &    78.7 &    5.01 &    55.6 &    4.73 &    40.4 &    4.74 \\
Fe\,I  &  5572.84 &  3.40 & $ -0.28$ & \nodata & \nodata &    49.3 &    4.80 &    32.5 &    4.57 & \nodata & \nodata \\
Fe\,I  &  5586.76 &  3.37 & $ -0.14$ &    45.3 &    4.68 &    59.8 &    4.80 &    47.4 &    4.66 & \nodata & \nodata \\
Fe\,I  &  5615.64 &  3.33 & $  0.05$ & \nodata & \nodata &    84.3 &    4.98 &    68.3 &    4.77 & \nodata & \nodata \\
Fe\,I  &  6065.48 &  2.61 & $ -1.41$ & \nodata & \nodata &    38.5 &    4.82 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6136.61 &  2.45 & $ -1.41$ &    20.9 &    4.41 & \nodata & \nodata &    34.2 &    4.63 & \nodata & \nodata \\
Fe\,I  &  6137.69 &  2.59 & $ -1.35$ &    28.6 &    4.69 &    47.5 &    4.89 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6191.56 &  2.43 & $ -1.42$ & \nodata & \nodata &    58.3 &    4.94 & \nodata & \nodata &    21.6 &    4.53 \\
Fe\,I  &  6230.72 &  2.56 & $ -1.28$ & \nodata & \nodata &    55.6 &    4.91 &    32.7 &    4.59 & \nodata & \nodata \\
Fe\,I  &  6252.56 &  2.40 & $ -1.69$ &    20.1 &    4.61 &    51.9 &    5.07 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6393.60 &  2.43 & $ -1.58$ & \nodata & \nodata & \nodata & \nodata &    28.6 &    4.66 & \nodata & \nodata \\
Fe\,I  &  6400.00 &  3.60 & $ -0.29$ &    18.7 &    4.50 &    40.4 &    4.85 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6421.35 &  2.28 & $ -2.01$ & \nodata & \nodata &    32.1 &    4.91 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6430.85 &  2.18 & $ -1.95$ & \nodata & \nodata &    44.4 &    4.95 &    19.5 &    4.53 & \nodata & \nodata \\
Fe\,I  &  6494.98 &  2.40 & $ -1.24$ &    33.9 &    4.46 &    76.3 &    5.00 &    36.0 &    4.42 & \nodata & \nodata \\
Fe\,I  &  6592.91 &  2.73 & $ -1.47$ &    21.2 &    4.77 &    35.9 &    4.95 & \nodata & \nodata & \nodata & \nodata \\
Fe\,I  &  6677.99 &  2.69 & $ -1.42$ & \nodata & \nodata &    45.8 &    5.02 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4178.86 &  2.58 & $ -2.51$ &    43.3 &    4.86 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4233.17 &  2.58 & $ -1.97$ &    68.8 &    4.78 &    75.2 &    4.72 &    61.7 &    4.53 &    52.1 &    4.69 \\
Fe\,II &  4416.82 &  2.78 & $ -2.60$ & \nodata & \nodata &    36.0 &    4.85 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4508.28 &  2.86 & $ -2.58$ &    15.2 &    4.58 &    39.8 &    4.99 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4515.34 &  2.84 & $ -2.60$ & \nodata & \nodata &    36.9 &    4.93 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4520.22 &  2.81 & $ -2.60$ & \nodata & \nodata &    34.7 &    4.86 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4522.63 &  2.84 & $ -2.25$ &    38.1 &    4.76 &    56.0 &    4.91 &    37.7 &    4.66 & \nodata & \nodata \\
Fe\,II &  4555.89 &  2.83 & $ -2.40$ & \nodata & \nodata &    48.4 &    4.92 & \nodata & \nodata & \nodata & \nodata \\
Fe\,II &  4583.84 &  2.81 & $ -1.93$ &    45.0 &    4.53 &    74.8 &    4.89 &    50.2 &    4.52 &    43.2 &    4.69 \\
Fe\,II &  4923.93 &  2.89 & $ -1.32$ &    70.3 &    4.44 &   103.1 &    4.89 &    84.6 &    4.59 &    62.1 &    4.52 \\
Fe\,II &  5018.45 &  2.89 & $ -1.22$ & \nodata & \nodata & \nodata & \nodata &    85.1 &    4.49 & \nodata & \nodata \\
Fe\,II &  5276.00 &  3.20 & $ -2.01$ &    25.1 &    4.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co\,I  &  3873.12 &  0.43 & $ -0.66$ & \nodata & \nodata &    66.8 &    2.10 &    61.7 &    2.11 & \nodata & \nodata \\
Co\,I  &  3995.31 &  0.92 & $ -0.22$ & \nodata & \nodata &    69.3 &    2.25 & \nodata & \nodata & \nodata & \nodata \\
Co\,I  &  4110.53 &  1.05 & $ -1.08$ & $<$81.0 & $<$3.69 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co\,I  &  4118.77 &  1.05 & $ -0.49$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & $<$66.3 & $<$3.03 \\
Co\,I  &  4121.32 &  0.92 & $ -0.32$ &$<$127.1 & $<$3.91 &    62.7 &    2.20 &    54.0 &    2.15 & \nodata & \nodata \\
Ni\,I  &  3783.52 &  0.42 & $ -1.42$ & \nodata & \nodata &   115.9 &    3.92 & \nodata & \nodata & \nodata & \nodata \\
Ni\,I  &  3858.30 &  0.42 & $ -0.95$ & \nodata & \nodata &   129.5 &    3.71 &   128.8 &    3.84 & \nodata & \nodata \\
Ni\,I  &  5080.52 &  3.65 & $  0.13$ & $<$49.7 & $<$4.52 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni\,I  &  5476.90 &  1.83 & $ -0.89$ & \nodata & \nodata &    88.8 &    4.00 &    64.5 &    3.65 & $<$81.1 & $<$4.34 \\
Sr\,II &  4077.71 &  0.00 & $  0.15$ &     syn & $<-1.89$&     syn & $<-2.16$&     syn & $<-1.85$&     syn & $<-1.20$\\
Ba\,II &  4554.03 &  0.00 & $  0.16$ &     syn & $<-2.18$&     syn & $<-2.15$&     syn & $<-2.14$&     syn & $<-1.99$\\
\enddata
\end{deluxetable*}

